CLEval: Character-Level Evaluation for Text Detection and Recognition Tasks

Despite the recent success of text detection and recognition methods, existing evaluation metrics fail to provide a fair and reliable comparison among those methods. In addition, there exists no end-to-end evaluation metric that takes characteristics of OCR tasks into account. Previous end-to-end metric contains cascaded errors from the binary scoring process applied in both detection and recognition tasks. Ignoring partially correct results raises a gap between quantitative and qualitative analysis, and prevents fine-grained assessment. Based on the fact that character is a key element of text, we hereby propose a Character-Level Evaluation metric (CLEval). In CLEval, the \textit{instance matching} process handles split and merge detection cases, and the \textit{scoring process} conducts character-level evaluation. By aggregating character-level scores, the CLEval metric provides a fine-grained evaluation of end-to-end results composed of the detection and recognition as well as individual evaluations for each module from the end-performance perspective. We believe that our metrics can play a key role in developing and analyzing state-of-the-art text detection and recognition methods. The evaluation code is publicly available at https://github.com/clovaai/CLEval.

==> multiline.tex <==
\begin{comment} %%% Multi-line comment out

% \sr{\bf{About Multiline Filtering}}\\
% \sr{ (1) 개인 질문 - Multiline 필터링이 end-to-end evaluation 측면에서 중요한 것인가요? }
% \ym{현재로선 그렇다고 생각합니다. Multiline으로 검출되면 인식 실패가 되니까요. 물론 satrn은 예외지만}\\
% \sr{ (2) orientation 정보가 없어서 폭비율 만으로 필터링한 것 같은데 사이드 효과는 없나요? }
% \ym{여기서는 폭비율 안씁니다. 좌상단 꼭지점이 시작점이기 때문에 orientation 정보는 있다고 볼 수 있습니다.}
% \sr{아! 이해 하였습니다.}\\
% \sr{(3) horizontally aligned 되어있다라는 가정이 있는 것인가요? }
% \ym{text box가 좌상단 꼭지점부터 시작이라고 하면 위의 가정 없이도 Multiline을 볼 수 이지 않나요?}
% \sr{이해 하였습니다.}\\
% \sr{(4) 좀 더 general 하게 위의 케이스가 이해시킬수 있는 방법은 없을까요? - 뭔가 edge case 가 존재 할 것 같은 느낌입니다.}
% \ym{네 동의합니다..... 좀더 고려해봐야겠네요.}

Although our instance matching policy works in a fairly generous way, there is a case when the match itself should be prevented. Multiline is a special case of many match involving multiple lines of texts and must be rejected by identifying it in the matching stage. 
\sr{Although our instance matching policy admits multiple pairs generously with a low standard, multiline text detection should be carefully treated with a high standard because the multiline text box have not been a target scenario in the text recognition stage. To prevent the edge cases, our matching process adopts an additional filtering methods, utilizing the orientation information of GT bounding boxes and relative angles between detected bounding boxes.}
Multiline detection is not favorable to recognition stage, so multiline prevention is third change of CLEval. This rejection involves not only many-to-one match where one detection contains multiple lines but also one-to-many match where multiple detections of different lines are matched to one GT.

\begin{figure}[t]
  \centering
  \includegraphics*[width=.5\linewidth, height=2.5cm, clip=true]{fig/multiline.png}
  \caption{Visualization of multiline computation. The angle $\theta$ satisfies Eq.~\ref{eq:ml-angle} and thus this match is rejected. \ym{그림 변경. 수식도 포함시키기} \sr{빈 공간을 활용하여 각도가 커졌을 때의 상황과 각도가 적을때의 상황을 예제로 보여주면 좋겠네요.}}
  \label{fig:ml}
  \vspace{-3mm}
\end{figure}

As shown in Fig.~\ref{fig:ml}, we use simple geometry to identify multiline. Firstly, define $B$ as a set of bounding boxes in the many side of a many match. Then we compute two pivotal points for all bounding boxes in $B$ by:
\begin{equation} \label{eq:ml-char}
\begin{gathered}
	{p_{i1}} = \text{mean}(v_{i1}, v_{i4}) \\
    {p_{i2}} = \text{mean}(v_{i1}, v_{i2}, v_{i3}, v_{i4})
\end{gathered}
\end{equation}
where $v_{ij}$ means the $j$th vertex $(x,y)$ of $B_i$. 
%Note that GT must assume the form of four vertices in a clockwise order starting from the top left point in regard to the orientation of the word.

The angle $\theta$ between $B_1$ and $B_2$ is then computed by turning from $p_{11}$ to $p_{12}$ around  $p_{22}$. While computing every possible angle among $B$, we reject the match when any one of it is:
\begin{equation} \label{eq:ml-angle}
    \left | min(\theta ,180-\theta ) \right |\geq 45^{\circ}.
\end{equation}
The threshold 45$^\circ$ is obtained experimentally.

% In addition, instead of selecting pivotal points as points on the edges, $p_{i1}$ is the point on the left edge and $p_{i2}$ is the center point of $B_i$. This is to make our algorithm robust against the width difference and distance between bounding boxes, which can confuse the magnitude of the angle. 

\sr{ \textbf{Suggestion:} Let $B$ be a set of source bounding boxes matched with a single target bounding box (i.e. one-to-many and many-to-one). Because characters in a line are aligned horizontally, the multiple text boxes covering the characters should be aligned in the same direction with the character sequence. To identify misaligned bounding boxes, we compute the center ($\textbf{p}^{\text{center}}_{b}$) and the medium point of the left edge($\textbf{p}^{\text{left}}_{b}$) for each bounding box, and then calculate the angle $\theta_{bb'}$ when showing two points, $\textbf{p}^{\text{center}}_{b}$ and $\textbf{p}^{\text{left}}_{b}$, from another center point, $\textbf{p}^{\text{center}}_{b'}$. Fig.~\ref{fig:ml} shows an example describing the angles. As can be seen, when $\theta_{bb'}$ increase, the probability of mis-alignment is also increasing. While computing every possible angle among $B$, we reject the match when 
\begin{equation} \label{eq:ml-angle}
    \text{max}_{b,b'\in B}\left | \text{min}(\theta_{bb'} ,180-\theta_{bb'} ) \right |\geq 45^{\circ}.
\end{equation}
The threshold 45$^\circ$ is obtained experimentally.}
\\ \sr{ (1) 45$^\circ$ 역시 이유가 필요할 것 같은데, 이유가 무엇일까요? Text Box들이 정 사각형이고 크기가 같으며 여백 없이 붙어 있는 상황이 45$^\circ$ 일 것 같은데 이 상황이 기준이 되는 이유가 몰까요? } 
\\ \sr{ (2) 개인 질문: 왜 왼쪽 중점과의 중심점을 보는 것일까요? (오른쪽 중점은 중요하지 않나요?) }
\\ \sr{ (3) 제안: 이 역시 PCC를 이용하는 방법은 없을까요? }

% \sr{ \textbf{(1)} $B$ 내부에 여러 pair를 만들수 있을꺼 같은데 그중 하나라도 threshold를 넘으면 필터링 되는 거죠? $ \text{max}_{b' \in B} \left | min(\theta_{bb'} ,180-\theta_{bb'} ) \right |\geq 45^{\circ}$}\\
% \sr{ \textbf{(2)} $\theta_{bb'}$ 을 bounding box $b$ 센터입장에서 bounding box $b'$의 두점의 각도로 정의를 한다고 하였을 때, 필터링 대상이 되는 것은 $b'$ 일까요 $b$ 일까요?}
\end{comment}

